PowerQuant: Automorphism Search for Non-Uniform Quantization

Deep neural networks (DNNs) are nowadays ubiquitous in many domains such as computer vision. However, due to their high latency, the deployment of DNNs hinges on the development of compression techniques such as quantization which consists in lowering the number of bits used to encode the weights and activations. Growing concerns for privacy and security have motivated the development of data-free techniques, at the expanse of accuracy. In this paper, we identity the uniformity of the quantization operator as a limitation of existing approaches, and propose a data-free non-uniform method. More specifically, we argue that to be readily usable without dedicated hardware and implementation, non-uniform quantization shall not change the nature of the mathematical operations performed by the DNN. This leads to search among the continuous automorphisms of $(\mathbb{R}_+^*,\times)$, which boils down to the power functions defined by their exponent. To find this parameter, we propose to optimize the reconstruction error of each layer: in particular, we show that this procedure is locally convex and admits a unique solution. At inference time, we show that our approach, dubbed PowerQuant, only require simple modifications in the quantized DNN activation functions. As such, with only negligible overhead, it significantly outperforms existing methods in a variety of configurations.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/experiments.tex <==
\section{Experiments}
\subsection{Datasets and Implementation Details}
We validate the proposed method on the image classification task of ImageNet \cite{imagenet_cvpr09} ($\approx 1.2$M images train/50k test).
In our experiments we used pre-trained MobileNets \cite{sandler2018MobileNetV2}, ResNets \cite{he2016deep}, EfficientNets \cite{tan2019efficientnet} and DenseNets \cite{huang2017densely}. We used Tensorflow implementations of the baseline models from the official repository.
The pre-trained networks achieve standard baseline accuracies on each tasks.
The quantization process was done using the Numpy python's library. Activations are quantized as unsigned integers and weights are quantized using a symmetric representation.

In our study, we performed the ablation using the uniform quantization operator over weight values from \cite{krishnamoorthi2018quantizing} and logarithmic quantization from \cite{miyashita2016convolutional}. For our comparison with state-of-the-art approaches in data-free quantization, we implemented the more complex quantization operator from SQuant \cite{squant2022} and matched their results on common benchmarks.

In the following sections, we validate the empirical properties of the method. First, we show the strong anti correlation between the reconstruction error and the accuracy of the quantized model which motivates its use as a proxy to fit the power parameter $a$. Second, we study the computational cost of the proposed quantization operator as compared to the uniform operator. Third, we provide a thorough comparison with existing data-free quantization method in order to demonstrate the outstanding results achieved by the proposed method.

\subsection{Parameter Fitting}
Fig \ref{fig:anti_correlation} illustrates the evolution of both accuracy and the reconstruction error as functions of $a$. Our target is the highest accuracy with respect to the value of $a$. However, in the data-free context, we only have access to the reconstruction error. Fortunately, as shown in our empirical results, we observed a very strong anti correlation. By minimizing the reconstruction error we reach the highest accuracy in every configurations. The minimization can't be performed using standard gradient descent as the rounding operation induces zero-valued gradients. Nonetheless, while the reconstruction curve is not convex, it is continuity and locally convex and admits a unique minimum. Thus, in practice, if we initialize the search within $[0;1]$ the reconstruction error is convex on this interval, which ensures convergence of the method with a simplex-based optimization method such as the Nelder-Mead algorithm.

Empirically, optimal values of $a$ are centered on $0.55$ which corresponds to the first distribution in Fig \ref{fig:quantized_distributions}. The optimal value $a$ is relatively stable for the easier quantization configurations (e.g. int8 and int6) but can introduce strong variations in accuracy on low bit quantization (e.g. ResNet 50 with int4 quantization). This shows the importance of optimising $a$ for each network and configuration over the use of a default value.
Furthermore, our results provide a novel insight on the difference between pruning and quantization. In unstructured pruning, the baseline method consists in setting to zero the smallest scalar weight values and keeping unchanged the highest non-zero values. This is similar to our proposed power quantization for $a > 1$, which zeroes-out most small scalar values and keeps the precision on large values. However, in practice, better accuracy is achieved using $a < 1$ which suggests that the assumptions behind unstructured pruning can't be applied to quantization in a straight forward manner. In quantization, without re-training, we have to focus on the majority of scalar weight values rather than larger scalar weight values.

\begin{figure}[!t]
    \centering
    \includegraphics[width = \linewidth]{figs/anti_correlation.pdf}
    \caption{Anti correlation between the accuracy and reconstruction error for several quantization configurations (int8, int6 and int4) and architectures (ResNet 50 and DenseNet 121).}
    \label{fig:anti_correlation}
\end{figure}

Another approach that puts more emphasis on the nuances between low valued weights is logarithmic based non-uniform quantization, which consists in mapping the continuous values to a discreet logarithmic distribution \cite{miyashita2016convolutional,zhou2017incremental}. In table \ref{tab:comparison_log_unif_power}, we compare the proposed power method to both uniform and logarithmic approaches. By definition the proposed power method significantly outperforms the uniform method in every scenario as the search space includes the uniform method, thus the optimal power solution is necessarily more accurate. Furthermore, it appears that the proposed methods systematically achieves a lower reconstruction error, which indicates a better fit to the weight distribution. This translates to a higher accuracy on every setup. More precisely, in int4, the proposed method improves the accuracy by 13.22 and 13.21 points on ResNet 50 and DenseNet 121 respectively. This improvement can also be attributed to a better quantization of the inputs of each layers, especially on ResNet 50 where the gap in the reconstruction error (over the weights) is relatively small. On a side note, the poor performance of the logarithmic approach on DenseNet 121 is attributed to the skewness of the weight distributions. Formally, ResNet 50 and DenseNet 121 weight values show similar average standard deviations across layers ($0.0246$ and $0.0264$ respectively) as well as similar kurtosis ($6.905$ and $6.870$ respectively). However their skewness are significantly different: $0.238$ for ResNet 50 and more than twice as much for DenseNet 121, with $0.489$. The logarithmic quantization, that focuses on very small value is very sensible to asymmetry which explains the poor performance on DenseNet 121. In contrast, the proposed method offers a robust performance in all situations.

\input{tables/log}

These results demonstrate the added value of the proposed power function based quantization as compared to other schemes. In order to provide a complete evaluation of the method, we evaluate two other aspects of the method. First, we empirically demonstrate that compared to uniform quantization, the proposed method doesn't harm the inference speed by modifying the activation functions. Second, we validate the performance of the method as quantization scheme with respect to other recent data-free quantization methods.

\subsection{Inference Cost and Processing Time}
Table \ref{tab:chorno} lists the difference in terms of inference time induced by the proposed method. This corresponds to the measurement of the added runtime attributable solely to a change in the activation function. For MobileNet, ResNet and MobileNet V2, the baseline activation function is the ReLU. This activation function is particularly fast to compute due to its simplicity. By performing the power quantization ,the ReLU activation functions becomes $x \mapsto |x|^a$ which is necessarily more time consuming to compute. In practice, our results show that this cost amounts to less than $1\%$ of the whole inference time on most networks. More precisely, in the case of ResNet 50, the change in activation function induces a slowdown of $0.15\%$. The exception is DenseNet with an increase of 3.4\% in runtime that is still negligible.

\input{tables/chrono}

Similarly, we measure the empirical time required to perform the proposed quantization method on several neural networks and report the results in table \ref{tab:process_time}. These result show that the proposed method offers outstanding trade-offs in terms of compression and accuracy at virtually no cost over the processing and inference time as compared to other data-free quantization methods. For instance, SQuant is a sophisticated method that requires heavy lifting in order to efficiently process a neural network. On a CPU, it requires at least 100 times more time to reach a lower accuracy than the proposed method as we will showcase in our comparison to state-of-the-art quantization schemes.

\input{tables/process_time}

\subsection{Comparison with Data-Free Quantization Methods}
In our comparison with other data-free quantization method, we add several known quantization stratagems in order to exploit the proposed method to its fullest. First, we incorporate bias correction from \cite{nagel2019data} which measures the expected difference between the outputs of the original and quantized models and updates the biases terms to compensate for this difference. 

In table \ref{tab:comparison_sota_resnet}, we report the performance of several data-free quantization scheme on ResNet 50. Although, no training data is involved in these process, some approaches such as ZeroQ \cite{cai2020zeroq} need data generation (DG) in order to calibrate parameters of the method. Furthermore, DSG \cite{zhang2021diversifying} and GDFQ \cite{xu2020generative} use the generated data for fine-tuning (FT), which restores the lost accuracy from a less efficient quantization operator. As shown, in standard quantization range (W8/A8), the proposed method greatly outperforms other data-free solutions. The gap is even wider on the challenging low bit quantization (W4/A4) where the proposed method improves the accuracy by almost two points over SQuant \cite{squant2022} which already restores the accuracy significantly better than GDFQ (by 12.95 points). This shows the effectiveness of the method on ResNet 50.

\input{tables/resnet}

In table \ref{tab:comparison_sota_densenet}, we report the performance of other data-free quantization processes on DenseNet 121. The OMSE method \cite{choukroun2019low} is a post-training quantization method, that leverages a sample validation sample during quantization. Consequently, it is not data-free. Yet, we include this work in our comparison as they show strong performance in terms of accuracy at a very low usage of real data. As shown, the proposed method almost restores the full-precision accuracy in W8/A8 quantization which offers a low improvement as compared to other sophisticated methods. On the other hand, on the challenging int4 quantization, methods such as SQuant lose over 23 points in accuracy. The proposed method improves the accuracy by 17.54 points over SQuant and by a remarkable 12.30 points over OMSE. 

\input{tables/densenet}

==> sections/methodo.tex <==
\section{Methodology}
Let $F$ be a trained neural network with $L$ layers each comprising a weight tensor $W_l$.
Let $Q$ be a quantization operator such that $Q(W_l)$ is represented on $b$ bits. Assuming a bell-shaped distribution, the standard approach for non-uniform quantization consists in applying a logarithmic distribution where the quantization steps increase exponentially
instead of linearly. In order to exploit such quantization, the quantized multiplications are overwritten using bit-shift operations instead of integer arithmetic. Furthermore these methods have limited adaptability as the increment speed is usually manually set. 

Taking aside the rounding operation in quantization, we want to define the space $\mathcal{Q}$ of functions $Q$ such that
\begin{equation}\label{eq:main}
    \forall Q \in \mathcal{Q}, \exists Q^{-1} \in \mathcal{Q} \quad \forall x,y \quad Q^{-1}(Q(x)*Q(y)) = x\times y
    \label{equ1}
\end{equation}
where $*$ is the intern composition law of the quantized space and $\times$ is the standard multiplication.
These functions encapsulated with the rounding operation will define our novel quantization operator. The proposed method will consist in the search of the best suited operator for a given set of trained neural network and input statistics.

\subsection{Automorphisms of $(R_+^*,\times)$}
Let $Q$ be a transformation from $\mathbb{R}_+$ to $\mathbb{R}_+$ such that for all $x,y \in \mathbb{R}_+^2$ we have $*$ is the multiplication and $Q(x)\times Q(y)=Q(x\times y)$. In order to have a de-quantization operation, we need $Q^{-1}$ to be defined \textit{i.e.} $Q$ is bijective. Thus $Q$ is a group automorphism of $(R_+^*,\times)$. Consequently, we have
\begin{equation}
    \begin{cases}
    \forall x\in \mathbb{R}_+, \quad Q(x)\times Q(0) = Q(0)\\
    \forall x\in \mathbb{R}_+, \quad Q(x)\times Q(1) = Q(x)\\
    \end{cases}
\end{equation}
which induces that $Q$ is either the constant $1$ or $Q(0)=0$ and $Q(1)=1$. Because $Q$ is an automorphism we can eliminate the first option. Now, we will demonstrate that $Q$ is necessarily a power function. Let $n$ be an integer, then 
\begin{equation}
    Q(x^n)=Q(x)\times Q(x^{n-1})=Q(x)^2\times Q(x^{n-2})=\dots= Q(x)^n
\end{equation}
Similarly, for fractions, we get
\begin{equation}
    Q(x^{\frac{1}{n}}) \times \dots \times Q(x^{\frac{1}{n}}) = Q(x) \Leftrightarrow Q(x^{\frac{1}{n}})=Q(x)^{\frac{1}{n}}
\end{equation}
Assuming $Q$ is continuous, we deduce that for any rational $a\in\mathbb{R}$, we have
\begin{equation}\label{eq:power_func_property}
    Q(x^a) = Q(x)^a
\end{equation}
In order to verify that the solution is limited to power functions, we use a \textit{reductio ad absurdum}.
Assume $Q$ is not a power function. Therefore, there exists $(x,y)\in\mathbb{R}_+^2$ and $a \in \mathbb{R}$ such that $Q(x)\neq x^a$ and $Q(y)=y^a$. By definition of the logarithm, there exists $b$ such that $x^b=y$. We get the following contradiction, from \ref{eq:power_func_property},
\begin{equation}
\begin{cases}
    Q({x^b}^a) = Q(y^a) = y^a\\
    Q({x^b}^a) = Q({x^a}^b) = {Q(x^a)}^b \neq \left({x^a}^b = y^a\right)
\end{cases}
\end{equation}
Consequently, the suited functions $Q$ are limited to power functions \textit{i.e.} $\mathcal{Q} = \{Q : x \mapsto x^a | a \in \mathbb{R}\}$.
For the sake of clarity, we will now include the rounding operation in the quantization operators.
\begin{equation}\label{eq:quantization_operator}
    \mathcal{Q} = \left\{ Q_a : W \mapsto \left\lfloor (2^{b-1}-1)\frac{\text{sign}(W)\times |W|^a}{\max{|W|^a}} \right\rfloor \Big| a \in \mathbb{R} \right\}
\end{equation}
Consequently, the operator $Q_a$ is not a bijection anymore and $Q^{-1}_a$ is no longer the inverse bijection. Thus, quantization introduces an error called, reconstruction error, defined as
\begin{equation}\label{eq:reconstruction_error}
    \sum_{l=1}^L \left\| W_l - Q_a^{-1}(Q_a(W_l)) \right\|_p
\end{equation}
The reconstruction error on the weights can be computed in a data-free context, contrary to the reconstruction error of the activations.
In order to quantize a neural network, we need to find a suitable value of $a$. To do so, we exploit the reconstruction error as a proxy.

\subsection{Weights Quantization and Minimization Problem}
We search in the space $\mathcal{Q}$ by solving the reconstruction error minimization problem defined as
\begin{equation}\label{eq:min_problem}
    \min_a\left\{ \text{error}(F, a) \right\} = \min_a\left\{ \sum_{l=1}^L \left\| W_l - Q_a^{-1}(Q_a(W_l)) \right\|_p \right\}
\end{equation}
where $\|\cdot\|_p$ is the $L^p$ norm (in practice $p=1$) and the $Q_a^{-1}$ operator is simply 
\begin{equation}
    Q_a^{-1}(W) = \text{sign}(W) \times \left|W \times \frac{\max{|W|}}{2^{b-1}-1}\right|^{\frac{1}{a}}
\end{equation}
which can be performed simultaneously with the activation function. In practice, this minimization problem is not convex but is locally convex and has a unique minimum and no plateau. We find the optimal value for $a$, using the Nelder–Mead method \cite{nelder1965simplex} which solves problems for which derivatives may not be known or, in our case, are not informative. More modern solvers are not required in order to reach the optimal solution. The weight quantization process is summarized in Algorithm \ref{alg:weights}. 
\begin{figure}[!t]
    \centering
    \includegraphics[width = \linewidth]{figs/quantized_distribs.pdf}
    \caption{Influence of the power parameter $a$ on the quantized distribution associated to a Gaussian prior. In such instance, the reconstruction error is minimized for $a < 1$.}
    \label{fig:quantized_distributions}
\end{figure}

We propose the following interpretation of the value of parameter $a$ based on Fig \ref{fig:quantized_distributions}. Uniform quantization and $a=1$ are equivalent and correspond to a quantization invariant to the weight distribution. For $a < 1$, the quantization is more fine-grained on weight values with low absolute value and coarse on high absolute values. To the contrary, for $a > 1$, the quantization is fine-grained on high absolute values. Intuitively, for centered and mono-modal distributions such as a standard Gaussian, the optimal value of $a$ with respect to equation \ref{eq:min_problem} will be below $1$. This corresponds to the observed situation.

On the other hand, inputs and activations quantization require a work around as their distribution is not available in the context of data-free quantization. Instead of generating synthetic images, we exploit statistics stored in the batch-normalization layers parameters.

\begin{algorithm}
\caption{Weight Quantization Algorithm}\label{alg:weights}
\begin{algorithmic}
\Require trained neural network $F$ with $L$ layers to quantize, number of bits $b$
\State $a \leftarrow$ solver($\min\{\text{error}(F, a)\}$)\Comment{in practice we use the Nelder–Mead method}
\For{$l \in\{1,\dots,L\}$}
    \State $W_{\text{sign}} \leftarrow \text{sign}(W_l)$ \Comment{save the sign of the scalar values in $W$}
    \State $W_l \leftarrow W_{\text{sign}} \times |W_l|^a$ \Comment{power transformation}
    \State $s \leftarrow \frac{\max{|W_l|}}{2^{b-1}-1}$ \Comment{get quantization scale}
    \State $Q(W_l) W_l \mapsto \left\lfloor\frac{W_l}{s}\right\rceil$ \Comment{quantization by rounding}
    \State $Q^{-1} W \mapsto W_{\text{sign}} \times |W \times s|^{\frac{1}{a}}$ \Comment{definition of the de-quantization operation}
\EndFor
\end{algorithmic}
\end{algorithm}

\subsection{Inputs Quantization Formulation}\label{sec:input_quantif}
Assume, their is a batch-normalization (BN) layer before a layer $l$ to quantize. We note $\beta$ and $\gamma$ the centering and scaling parameters of the BN layer. Consequently, on a trained neural network $F$ of domain $\mathcal{D}$, we can assert that
\begin{equation}\label{eq:stats}
    \mathbb{E}_{X\in\mathcal{D}}[\text{Input of layer } l] = \beta \quad \text{and} \quad \mathbb{V}_{X\in\mathcal{D}}[\text{Input of layer } l] = \gamma^2
\end{equation}
In order to apply algorithm \ref{alg:weights} to the inputs we need to tackle three challenges. First, we don't want to store the signs of the inputs which will change at each inference. This is solved by assuming that the network uses ReLU activation functions. Second, we need to find a suitable value for parameter $a$. Furthermore, we need to select one value for $a$ to use on both weights and inputs in order to satisfy the hypothesis from equation \ref{eq:main}. Fortunately, in practice, the values that fit the weight distribution also provide a good quantization of the inputs.

==> sections/related.tex <==
\section{Related Work}
\subsection{Quantization}
In this section, we provide a background on the current state of DNNs quantization. Notice that while certain approaches are geared towards memory footprint reduction (e.g. without quantizing inputs and activations) \citep{chen2015compressing,gong2014compressing,han2015deep,zhou2017incremental}, in what follows, we essentially focus on methods that aim at reducing the inference time. In particular, motivated by the growing concerns for privacy and security, data-free quantization methods \citep{banner2019post,cai2020zeroq,choukroun2019low,fang2020post,garg2021confounding,zhao2019improving,nagel2019data,squant2022} are emerging and have significantly improved over the recent years. 

The first breakthrough in data-free quantization \citep{nagel2019data} was based on two mathematical ingenuities. First, they exploited the mathematical properties of piece-wise affine activation functions (such as e.g. ReLU based DNNs) in order to balance the per-channel weight distributions by iteratively applying scaling factors to consecutive layers. Second, they proposed a bias correction scheme that consists in updating the bias terms of the layers with the difference between the expected quantized prediction and the original predictions. They achieved near full-precision accuracy in int8 quantization. Since this seminal work, two main categories of data-free quantization methods have emerged. First, data-generation based methods, such as \cite{cai2020zeroq,garg2021confounding}, that used samples generated by Generative Adversarial Networks (GANs) \citep{goodfellow2014generative} as samples to fine-tune the quantized model through knowledge distillation \citep{hinton2015distilling}. Nevertheless, these methods are time-consuming and require significantly more computational resources. Other methods, such as \cite{banner2019post,choukroun2019low,fang2020post,zhao2019improving,nagel2019data,squant2022}, focus on improving the quantization operator but usually achieve lower accuracy. One limitation of these approaches is that they are essentially restricted to uniform quantization, while considering non-uniform mappings between the floating point and low-bit representation might be key to superior performance.

\subsection{Non-Uniform Quantization}
Indeed, in uniform settings, continuous variables are mapped to an equally-spaced grid in the original, floating point space. Such mapping introduces an error: however, applying such uniform mapping to an \textit{a priori} non-uniform weight distribution is likely to be suboptimal in the general case. To circumvent this limitation, non-uniform quantization has been introduced \citep{banner2019post,hubara2016binarized,jeon2020biqgemm,wu2016quantized,zhang2018lq,miyashita2016convolutional,zhou2017incremental}. We distinguish two categories of non-uniform quantization approaches. First, methods that introduce a code-base and require very sophisticated implementations for actual inference benefits such as \cite{banner2019post,hubara2016binarized,jeon2020biqgemm,wu2016quantized,zhang2018lq}. Second, methods that simply modify the quantization operator such as \cite{miyashita2016convolutional,zhou2017incremental}. In particular, \cite{miyashita2016convolutional} proposes a log-quantization technique where multiplications are replaced by bit shifts. Nevertheless, one limitation of this approach is that because the very nature of the mathematical operations is intrinsically altered, in practice, it is hard to leverage without dedicated hardware and implementation. 
\revision{Instead of transforming floating point multiplications in integer multiplications, they change floating point multiplications into bit-shifts or even look up tables (LUTs). Some of these operations are very specific to some hardware (e.g. LUTs are thought for FPGAs) and may not be well supported on most hardware. Conversely, in this work, we propose a non-uniform quantization scheme that preserves the nature of the mathematical operations by mapping floating point multiplications to standard integer multiplications.} As a result, our approach \revision{boils down} to simple modifications of the computations in the quantized DNN, hence allowing higher accuracies than uniform quantization methods while leading to straightforward, ready-to-use inference speed gains.
Below we describe the methodology behind the proposed approach.

==> tables/solvers.tex <==
\begin{table}[!t]
\caption{Comparison between the proposed estimation of $a$ based on the reconstruction error (R.E.) from equation \ref{eq:reconstruction_error} and other metrics based on white noise (W.I.), deep inversion (D.I.) or real images (R.I.).}
\label{tab:solvers}
\centering
\setlength\tabcolsep{4pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
Architecture & Method & W-bit & A-bit & accuracy & W-bit & A-bit & accuracy \\
\hline
\hline
\multirow{4}{*}{MobileNet V2}
 & R.E. & 6 & 6 & 69.104 & 4 & 4 & 36.0 \\
 & W.N. & 6 & 6 & 69.578 & 4 & 4 & 17.8 \\
 & D.I. & 6 & 6 & 69.671 & 4 & 4 & 9.59 \\
 & R.I. & 6 & 6 & 70.120 & 4 & 4 & 41.6 \\
\hline
\end{tabular}
\end{table}
